CoMeta: Enhancing Meta Embeddings with Collaborative Information in Cold-start Problem of Recommendation

The cold-start problem is quite challenging for existing recommendation models. Specifically, for the new items with only a few interactions, their ID embeddings are trained inadequately, leading to poor recommendation performance. Some recent studies introduce meta learning to solve the cold-start problem by generating meta embeddings for new items as their initial ID embeddings. However, we argue that the capability of these methods is limited, because they mainly utilize item attribute features which only contain little information, but ignore the useful collaborative information contained in the ID embeddings of users and old items. To tackle this issue, we propose CoMeta to enhance the meta embeddings with the collaborative information. CoMeta consists of two submodules: B-EG and S-EG. Specifically, for a new item: B-EG calculates the similarity-based weighted sum of the ID embeddings of old items as its base embedding; S-EG generates its shift embedding not only with its attribute features but also with the average ID embedding of the users who interacted with it. The final meta embedding is obtained by adding up the base embedding and the shift embedding. We conduct extensive experiments on two public datasets. The experimental results demonstrate both the effectiveness and the compatibility of CoMeta.

==> section/preliminaries.tex <==
\begin{figure}
    \centering
	\includegraphics[width=0.9\linewidth]{figure/fig1-v2.pdf} 
	\caption{General architecture of recent recommendation models.}
	\label{fig:1} 
\end{figure}

\section{Preliminaries}
Without the loss of generality, in this paper we mainly focus on binary classification recommendation tasks, such as CTR prediction.
For both users and items, their features consist of their IDs and their attribute features (\textit{e.g.}, age and occupation for users, category and price for items).
The sample $\{i,j,y\}$ indicates the interaction between user $i$ and item $j$, where the label $y\in\{0,1\}$ is the user feedback.
As illustrated in Figure \ref{fig:1}, most recent recommendation models~\cite{song2019autoint} follow the framework as below:

\textbf{Input layer.}
The model inputs are user features and item features.

\textbf{Embedding layer.}
Embedding techniques can transform the raw features into dense vectors.
For user $i$, we suppose $\mathbf{u}_i$ is the user's ID embedding and 
$\mathbf{Z}_i = \left \{ \mathbf{Z}_{i}^{1}, \mathbf{Z}_{i}^{2} , \cdots , \mathbf{Z}_{i}^{n} \right \}$ 
is the set of the user's attribute feature embeddings, where $n$ denotes the number of user attribute features.
Similarly, we have an item ID embedding $\mathbf{v}_j$ and a set of item attribute feature embeddings
$\mathbf{Z}_j = \left \{ \mathbf{Z}_{j}^{1}, \mathbf{Z}_{j}^{2} , \cdots , \mathbf{Z}_{j}^{m} \right \}$ 
for item $j$, where $m$ denotes the number of item attribute features.
The embedding of each sample can be expressed as:
\begin{equation}
    \mathbf{E} = \left [ \mathbf{u}_i , \mathbf{Z}_i , \mathbf{v}_j , \mathbf{Z}_j \right ].
\end{equation}

\textbf{Hidden layers.}
In the hidden layers (usually a MLP) that capture the high-order interactions with non-linearity, the long embedding vector $\mathbf{E}$ is transformed into a compact representation as:
\begin{equation}
    \mathbf{s} = MLP\left ( \mathbf{E} \right ) = MLP\left ( \mathbf{u}_i , \mathbf{Z}_i , \mathbf{v}_j , \mathbf{Z}_j \right ).
\end{equation}

\textbf{Prediction layer.}
The prediction layer, which consists of a linear layer and an active layer, makes the final prediction as:
\begin{equation}
    \hat{y} = \sigma \left ( \mathbf{Ws} + \mathbf{b} \right ),
\end{equation}
where $\hat y \in \left [ 0 , 1 \right ]$ is the final prediction; $\sigma \left ( \cdot \right )$ is the sigmoid function; $\mathbf{W}$ and $\mathbf{b}$ are learnable parameters (\textit{i.e.}, the weights and the bias) in the linear layer.

We adopt the cross-entropy loss, the most widely used loss function for binary classification recommendation tasks, as our loss function:
\begin{equation}
    loss = -\frac{1}{N} \sum_{i=1}^{N} y_i \log \hat y_i + \left ( 1 - y_i \right ) \log \left ( 1-\hat y_i \right ),
\end{equation}

where $N$ is the number of training samples; $y_i$ is the label of the $i$-th sample; $\hat y_i$ is the prediction of the $i$-th sample.


